MEG Source Localization via Deep Learning

We present a deep learning solution to the problem of localization of magnetoencephalography (MEG) brain signals. The proposed deep model architectures are tuned for single and multiple time point MEG data, and can estimate varying numbers of dipole sources. Results from simulated MEG data on the cortical surface of a real human subject demonstrated improvements against the popular RAP-MUSIC localization algorithm in specific scenarios with varying SNR levels, inter-source correlation values, and number of sources. Importantly, the deep learning models had robust performance to forward model errors and a significant reduction in computation time, to a fraction of 1 ms, paving the way to real-time MEG source localization.

==> background_old.tex <==
% paragraph order
% 1. hydro expl + workflow + motivation
% 2. the solution + ML in geosciences context
% 3. seismic data
% 4. about the method pros + cons
% 5. vision



% our approach and ML in geoscience and how is helping exploration
This work proposes an alternative to the current exploration workflow which has the potential of dramatically speedup the decision process. Our approach is an end-to-end solution. Contrary to standard techniques such as seismic
tomography~\cite{Rawlinson2010}, it produces earth models directly from 
untreated seismic data. Seismic tomography is fundamentally equivalent to medical tomography. Further, our approach is competitive with wave equation-based modeling/inversion, in particular regarding computing costs and turnaround time. Key characteristics of our approach is the lack of human intervention and biases, and that it is fully automated. The former is not a minor point, domain experts are heavily involved during projects with many multi-weeks iterations in order to produce earth models. Given the current pervasive use of ML, some specific steps of the standard hydrocarbon exploration workflow (\cite{zhang2014,Duan2018,Mandelli2019}) are being replaced by data-driven methods. Nonetheless, most of the advances happen on the interpretation (\cite{Di2018}) of the earth models rather than in the generation of them.

% about seismic data description


% pros and cons of the approach
The general Deep Learning approach taken in this work 
follows recent developments described in \cite{dahlke2016, Araya2018, Farris2018} (and others fully described in Section~\ref{sec:related}), the connecting element is the use of untreated seismic data, something rarely attempted for the tasks described. Commonly seismic data is subjected to partial differential equations (PDE)-based modeling/inversion in order to solve the among mentioned tasks. The core of the supervised DL approach is the use of statistical models to map untreated input seismic data (or extracted features from it) directly to the final desired earth model (or desired derivatives) in 2D or 3D. A key element of our method is the use of Spectrogram images as input features, computed from seismic data (see in Fig.~\ref{fig:survey} referred as traces). These Spectrograms reveal temporal changes in the spectral content of seismic traces. This feature extraction step is automated and not subjected to human bias. Another advantage of this approach relates to  and shared with all DL applications, is that the computing costs are all one-off payed upfront. After training, velocity 
model (main earth model aspect cover in this work) reconstruction computational costs are negligible, thus making the overall 
computing requirements a fraction of those needed for traditional techniques, in particular the ones involving partial PDE-based solutions.
The main concerns, common to many DL-based applications, are: access to proper amount and quality labels and generalization power of the trained models. The former is addressed by synthetic modeling generation, which is in our case is complemented with salt body structures extracted from deployed velocity models. The later basically set the limits of how much a predicting model can accurately predict from unseen data, it is currently an open field of research, and therefore we can only propose speculative ideas about it. 

We envision this approach as a facilitator for advanced model reconstruction as early as during the data acquisition campaigns, where domain experts can performing online scenarios testing when feeding back their model modifications. Therefore, the domain experts at back to the center of the critical decision making process and not just focused in cumbersome data oriented tasks. Finally, this approach and similar 
can also enhanced other geoscience applications such as seismology, shallow hazards, planetary exploration, etc. 




==> outline.tex <==

\begin{figure*}[ht]
\centering
\includegraphics[width=0.85\textwidth]{figs/MEG_Forward_Inverse.png}
\caption{MEG forward and inverse problems: in the forward problem a well-posed model maps the true sources activation to the MEG measurement vector. In the inverse (and ill-posed) problem, an inverse operator maps the measurement vector to the estimated sources activation.}
\label{fig:forward_inverse}
\end{figure*}
The proposed manuscript will include five sections, constituting a self-contained  paper, as detailed in the following.


This section will describe the motivation and significance of MEG source localization for neurorehabilitation and BMI, expanding the explanation in section III above. The successful utilization of DL for achieving state-of-the-art results in numerous inverse problems will be discussed, thus motivating to use DL for MEG source localization. In addition, essential physical definitions and explanations of MEG signals will be provided, and the associated forward and inverse problems will be formulated. The forward problem is given by:
\begin{equation}
    \mathbf{y}_t=\mathbf{M}\mathbf{q}_t+\mathbf{n}_t,
\end{equation}
where $\mathbf{y}_t$ is the time-dependent MEG measurement vector, $\mathbf{M}$ is the time-invariant gain matrix, computed for a given 3D brain model, $\mathbf{q}_t$ is the time-dependent sources activation's vector and $\mathbf{n}_t$ is a time-dependent noise vector. The inverse problem aims to estimate the true sources activation's, which encode the sources locations, from the noisy measurement $\mathbf{y}_t$:
\begin{equation}
    \hat{\mathbf{q}}_t=\mathbf{T}(\mathbf{y}_t),
\end{equation}
where $\mathbf{T}()$ is the inversion operator which maps data from the measurement space to the localization space. Fig. \ref{fig:forward_inverse} illustrates the relation between the forward and inverse problems.
\subsection{Overview of MEG Source Localization Methods (1 page)}
This section will explain the main approaches and limitations of existing MEG/EEG source localization methods. The spatial resolution of MEG/EEG is limited since the inverse problem of estimating the sources of extracranial signals is ill-posed: different current distributions that can explain similar data, and the solutions are therefore sensitive to noise. Many methods have been developed to localize brain activity using different anatomically and physiologically meaningful constraints, which render the solution unique. The most common approaches include minimum-norm estimate (MNE) \cite{NME1994}, dynamic statistical parametric mapping (dSPM) \cite{DALE200055}, standardized low-resolution
electromagnetic tomography (sLORETA) \cite{sLORETA}, beamforming \cite{HILLEBRAND2005149}, and multiple signal classification (MUSIC) \cite{740118,MAKELA201873}. However, a common problem in all these approaches is that they fail in the case of highly correlated sources, referred to as synchronous sources. Though several methods aimed at coping with synchronous sources have been developed, they either require some a-priori information on the location of the synchronous sources, are limited to the localization of pairs of synchronous sources, or are limited in their performance. These methods and limitations will be highlighted in this section.


\subsection{Deep Learning for MEG Source Localization (4 pages)}
This section will be the main constituent of the article, explaining in detail the proposed DL solutions and associated conceptual novelties. The following sub-sections will be included: (i) A brief review of relevant DL principles: network layers and activation functions, empirical risk minimization, gradient-based learning, and regularization. (ii) A description of the  training data generation workflow, which utilizes the MEG forward model. (iii) The proposed deep neural network (DNN)  solution illustrated in Fig. \ref{fig:DNN}, will be presented in detail, along with the architectural considerations, training procedures, and the computational advantages as compared to non-DL methods. (iv) the conceptual novelties provided by the DL solution will be discussed, including high localization accuracy with a single MEG snapshot, high localization accuracy with synchronous sources, and robustness to noise.\\
\begin{figure*}
\centering
\includegraphics[scale=0.5]{figs/MEG_DNN_Inverse.png}
\caption{Illustration of the DNN-based MEG source localization solution: the end-to-end inversion operator performs mapping from the MEG measurement space to the sources activation space.}
\label{fig:DNN}
\end{figure*}
\subsection{Performance Evaluation (3 pages)} 
The performance of the proposed methods will be thoroughly evaluated and compared against existing methods, in two scenarios: (1) the 3D cortex models of 5-10 human subjects, who participated in MEG experiments at the McGovern Institute of Brain Research, will be used to compute the corresponding forward models, and simulate millions of possible dipoles sources activation with several active dipoles (per human subject). (2) The Elekta Neuromag\footnote{\url{https://www.elekta.com/diagnostic-solutions/elekta-neuromag-triux}} phantom, depicted in Fig. \ref{fig:Elekta}, will be utilized to evaluate the performance. This phantom contains 32 artificial dipoles and five fixed head-position indicator coils. The phantom dipoles are energized using an internal signal generator. Only one dipole can be activated at a time, however, we will average data to simulate the simultaneous activation of multiple dipoles. The location of each dipole is recorded relative to the center of the sphere (0,0,0)m..  

\begin{figure}
\centering
\includegraphics[scale=1.05]{figs/Elekta.png}
\caption{The Elekta Neuromag phantom contains 32 artificial dipoles and five fixed head-position indicator coils. The phantom dipoles are energized using an internal signal generator.}
\label{fig:Elekta}
\end{figure}

\subsection{Conclusions (0.5 page)}
This section will highlight the solutions and results presented in the article, and summarize future research directions.

\begin{figure*}[H]
\centering
\includegraphics[scale=0.31]{figs/Forward_Inverse.png}
\caption{In the forward problem the seismic survey is performed to map the ground truth (and unknown) velocity model to recorded seismic data. The inverse problem is concerned with predicting the velocity model from the recorded seismic data. }
\label{fig:FORWARD_INVERSE}
\end{figure*}

==> related.tex <==
This section will be the main constituent of the article, explaining in detail the conceptual novelties provided by DL, and reviewing over 20 recent deep-learning-based solutions for seismic inverse problems, as detailed in Table \ref{tab:lit_survey}. 
\begin{comment}
In the context of Subsurface Model Building (VMB) for exploration geophysics, i.e., the search for subsurface models that honor the seismic recordings, the industry main approaches are Tomography and Full-waveform Inversion (FWI). Both of them developed through the years produced a large number of variations, in common they have the fact they are solving an ill-posed and ill-conditioned inverse problem. Lately, a Deep Learning (DL) approach was introduced by Araya-Polo et al. \cite{Araya2018}. In this section, no theoretical claims w.r.t. differences between the three approaches are introduced, and it only provides a review of the literature addressing DL as a solution to the VMB problem.    
\end{comment}
The literature covered in this section can be divided between works that mix elements of DL with classical methods (such as Full Waveform Inversion) (\cite{lewis17,Richardson18,Li2018,mosser2018,sun2018low}), and works that follow pure DL approaches to solve the above mentioned inverse problem (\cite{Kim18,Wang18,wu2018,Zheng18,Oye19,Li2019,Yang19,mao2019,ZhengTLE19}). Also, we have only selected works that appeared after the introduction of Deep Learning (circa 2016), therefore disregarding early attempts of using shallow Artificial Neural Networks.

\begin{comment}
In Lewis et al. \cite{lewis17}, it can observed the first attempt, that we are aware of, to use DL methods to assist FWI. A CNN-based network produces probability maps per iteration that help FWI to converge with higher accuracy when facing complex salt bodies. Further, Sun and Demanet \cite{sun2018low} addressed one well-known FWI drawback, lack of low-frequency information. They proposed a deep-learning-based bandwidth extension method. It is implemented as a regression task solved by an CNN architecture, this helps to setup a initialization step of FWI which usually is incomplete for lack of low-frequency content in the seismic record. In Li et al. \cite{Li2018}, the FWI iterative algorithm is augmented with a multiclass dictionary that learns from prior models, in this way helping to avoid local minimum, and therefore steering FWI convergence to high-quality results for well-known synthetics cases.

The work of Richarson \cite{Richardson18} is original and interesting: the FWI iterative process is re-written: firstly by using Recurrent Neural Networks (RNN) for synthetic data generation. Secondly, Automatic Differentiation (AD) and adjoint state method compute the gradient of the observed data and synthetic data misfit. Finally, the overall optimization process is solve by using Adam and Stochastic Gradient Descent method. Mosser et al. \cite{mosser2018} also reformulate the FWI in a way that barely resemble the original approach, the modeled data is generated from GAN-produced models, thus allowing a comprise representation by only a low dimension set of latent variables, then the numerical solution of the inversion misfit is obtained by using the adjoint method.

Alfarraj et al. \cite{alfarraj2018} and Das et al. \cite{das2018}, both work focus their attention to a related problem, which is the use of DL/ML based inversion to reconstruct impedance and density models.
% more to come

Wang et al. \cite{Wang18}, Zheng et al. \cite{Zheng18}, {\O}ye et al. \cite{Oye19}, Li et al. \cite{Li2019}, Yang et al. \cite{Yang19}, Zheng et al. \cite{ZhengTLE19} follow Araya-Polo et al. \cite{Araya2018} with only minor differences in DL architecture. A good portion of these references are very recent. The commonality is the use CNN layers as part of the neural network architectures, some of the them in sequences of encoders-autoencoders. Also, all of them are able to solve the VMB problem at least at the level of the FWI approach (Farris et al. \cite{Farris2018}). The other commonality is the use of mostly synthetic datasets, which indicates that approach is still on early research state, what follows is the use of field seismic recordings.

Kim et al. \cite{Kim18} starts as a general comparison of classical vs DL way of solving inverse problems with seismic data, but it focused on seismic reflectivity. Also, recently Russell \cite{RussellTLE19} presented a thorough comparison of classical and ML-based inversion approaches, in particular the analysis focused on quantitative and numerical issues.
\end{comment}
 


%What is missing in the field, and how it can be addressed. 
Main drawbacks of current approaches to VMB are two-fold: first, data related as lack of low frequency content of the field data, amplitude discrepancy \cite{li16} and cycle-skipping \cite{gang19}. Second, robustness of the iterative algorithms (stuck in local minimum) and methodological shortcomings from approximating the wave equation (\cite{zimmer19}). Data-driven approaches like DL will impacted by the same data shortcomings as the traditional approaches, but we expect gains on the methodological/algorithmic side. Also, specific DL techniques are under research to improve the data quality issues (for instance \cite{sun2018low}).

==> results.tex <==
The image quality of the proposed architectures was evaluated by generating a dataset of 12,000 velocity models of dimensions $70 \times 90$ grid points, with 4-8 layers, out of which 9,000 contain salt bodies. The velocity of the models ranges from 2000 to 4000[m/s], and of the salt bodies from 4450 to 4550[m/s]. From each velocity model, a seismic gather of $N =  N_S\times N_{R} = 153$ traces was generated by wave-based forward modelling, using $N_S = 3$ shots and $N_R = 51 $ receivers arranged in a linear array. The dataset split is 9,600 examples for training, 400 examples for validation, and 2,000 examples for testing. Each example consisting of a velocity model (the label) and the associated seismic gather (the data). Each network was implemented in TensorFlow, trained using the ADAM \cite{ADAM} optimizer over 50 epochs, a mini-batch size of 100, and with the mean squared error (MSE) as the loss function.  Table 2 compares the various network architectures in terms of the number of coefficients and image reconstruction quality, over 2,400 test models, as measured using the structural similarity SSIM \cite{Wang2004} and MSE. The performance was evaluated with noise levels of 10dB, 20dB and without noise.

\begin{table*}[H]
\caption{Evaluated Deep Networks Architectures}
\centering
\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|c|}
\hline
Input & Network & $1^{st}$ Layer &  $2^{nd}$ Layer & $3^{rd}$ Layer &$4^{th}$ Layer  & $5^{th}$ Layer & $6^{th}$ Layer & $7^{th}$ Layer  & $8^{th}$ Layer &  $9^{th}$ Layer \\
\hline
 Space-Frequency & CNN-SF  & Conv2D                     &  Maxpool        & FC             &  FC            &  FC            & Upsample             & Conv2D      & Conv2D     & Conv2D \\
       
 &  RNN-SF  & Conv2D            &  RNN(512)        & FC              & Upsample              & Conv2D            & Conv2D        & Conv2D            & -           & - \\
             
 &  LSTM-SF  & Conv2D             &  LSTM(512)       & FC             & Upsample              & Conv2D            & Conv2D        & Conv2D            & -           & - \\
                
 & GRU-SF   & Conv2D              &  GRU(512)        & FC             & Upsample              & Conv2D            & Conv2D        & Conv2D            & -           & - \\
                
\hline
Space-Time & CNN-ST     & Conv1D      &  Maxpool      &  FC            & FC         &  FC            & Upsample        & Conv2D        & Conv2D   & Conv2D \\
           & RNN-ST     & Conv1D      &  Maxpool      &  RNN(512)      & FC         & Upsample     & Conv2D            & Conv2D        & Conv2D   & -   \\
           & LSTM-ST    & Conv1D      &  Maxpool      &  LSTM(512)     & FC         & Upsample     & Conv2D            & Conv2D        & Conv2D   & -    \\
           & GRU-ST     & Conv1D      &  Maxpool      &  GRU(512)      & FC         & Upsample     & Conv2D            & Conv2D        & Conv2D   & -    \\
\hline
\end{tabular}
\label{tab:Architectures_Summary}
\end{table*}


\begin{table*}
\caption{Networks Comparison}
\centering
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
Architecture & CNN-SF &  RNN-SF & LSTM-SF & GRU-SF  & CNN-ST &  RNN-ST & LSTM-ST & GRU-ST \\
\hline
 Total number of coefficients  &  4,470,856    &  1,521,224       &   2,899,016     &  2,439,752
    &    3,418,120          & 1,648,136            & 2,731,016            &  2,370,056          \\
\hline
Number of coefficient in recurrent layer  &     &          &               &            &             &         &             & -         \\
\hline
Percentage of coefficients vs. CNN network  &             &         &              &              &             &         &             & -           \\
\hline
\end{tabular}
\end{table*}

\begin{table*}
\caption{Velocity Model Building Quality Comparison (averaged over 2,400 velocity models)}
\centering
\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|}
\hline
Noise Level & Metric & CNN-SF &  RNN-SF & LSTM-SF & GRU-SF  & CNN-ST &  RNN-ST & LSTM-ST & GRU-ST \\
\hline
SNR=10dB  & PSNR[dB]    &  28.2419    &     28.3091       &    28.4597          &  28.5197           &  28.1533          & 27.8169        & 28.2262           &  28.1598          \\
          & SSIM        &  0.8273           &  0.8204        &   0.8254         &  0.8222             &  0.8274           & 0.8218         & 0.8261            &  0.8244           \\
\hline
SNR=20dB  & PSNR[dB]    &   29.4343     &   29.1517          &  29.6410              &   29.3048             &     29.1816         &   29.3874           & 29.6825          &  29.6473           \\
          & SSIM        &   0.8380      &   0.8317           &     0.8431             &  0.8342              &   0.8365           &  0.8342              & 0.8419           &   0.8386           \\
\hline
Noiseless & PSNR[dB]    &    30.2601   &    29.9057     &  30.6745     &  30.6918                & 30.2483          & 30.2096        & 30.4596    & 30.5766          \\
          & SSIM        &     0.8479   &  0.8385        &  0.8537      &  0.8513                 & 0.8506           & 0.8433         & 0.8515     & 0.8509           \\
\hline
\end{tabular}
\end{table*}


==> tomo.tex <==
\begin{figure}
\includegraphics[trim= 50 50 0 0, clip, scale=0.675]{figs/VM.eps}
\caption{A two-dimensional velocity model: subsurface layers are modeled according to their acoustic wave propagation velocity in meters/seconds (m/s). Vertical axis (z) denotes depth, and horizontal axis (x) denotes lateral offset. }
\label{fig:VelocityModel}
\end{figure}
Subsurface Model Building can be understand as a tomography \cite{Rawlinson2010} of Earth (namely Seismic Tomography) based on seismic data recorded on the field. At its core is an inverse imaging problem, in which the observation model (subsurface model) can be represented as:
\begin{equation}
\mathbf{d}=\mathbf{F}(\mathbf{m})+\epsilon,
\end{equation}
where $\mathbf{d}$ is the observed (recorded) seismic data gather, $\mathbf{m}$ is the unknown velocity model, as depicted for example in Figure \ref{fig:VelocityModel}. $\mathbf{F}()$ is a mapping operator from the velocity model space to the seismic data space, and $\epsilon$ is ambient noise. The relation between the ground truth velocity model, and the associated forward and inverse problems is illustrated in Fig. ~\ref{fig:FORWARD_INVERSE}. 
\begin{figure*}
\centering
\includegraphics[scale=0.31]{figs/Forward_Inverse.png}
\caption{In the forward problem the seismic survey is performed to map the ground truth (and unknown) velocity model to recorded seismic data. The inverse problem is concerned with predicting the velocity model from the recorded seismic data. }
\label{fig:FORWARD_INVERSE}
\end{figure*}

The task of seismic tomography is to provide an estimate $\hat{\mathbf{m}}$ of the unknown velocity model $\mathbf{m}$, from the observed seismic data, and thus it approximates the inverse mapping operator $\mathbf{F}^{-1}()$.
Seismic tomography can be expressed as the solution to the following optimization  problem:
\begin{equation}
\hat{\mathbf{m}} = \arg \min_{\mathbf{m}}\sum_{i=1}^{N_{S}} ||\mathbf{d}_i^{pred} (\mathbf{m}) - \mathbf{d}^{obs} _i||_2^2,
\label{eq:tomo}
\end{equation}
where $V$ is the velocity model, depicted for example in Fig. \ref{fig:VelocityModel},  that minimizes $J(V)$, $d_V$ is a data vector that is modeled from a non-linear modeling operator $f(V)$, and $d_{obs}$ is the
recorded data vector. While it is common to minimize the sum of the squares
(represented here by the square of the L2 norm), other objective functions may
be used. Note that in the case of travel-time tomography the data vectors
contain travel-times (\cite{Scott1991}) that are modeled via the solution of the Eikonal equation.
Alternatively, in the full waveform inversion (FWI) (\cite{virieux2009}) case, the data contain the seismic 
records that are modeled via the numerical solution of the wave-equation. 
Solving this inverse problem, namely, finding the model that minimizes $J(\textbf{m})$, is notoriously difficult for a variety of reasons. Primarily, the objective function is nonlinear with respect to $\textbf{m}$, which means a perturbation in the earth model is not linearly mapped into the modeled data. It follows that the numerous, well studied strategies to solve linear least squares inverse problems are useless to us. Instead we must resort to nonlinear regression techniques for which there is no general theory for finding the optimal model parameters \cite{Aster}. Iterative methods are a popular choice for solving nonlinear inverse problems and rely on the gradient of the objective function at the current model iteration, $\textbf{m}_j$, to update the model parameters to find the next model iteration, $\textbf{m}_{j+1}$. 

\begin{equation}
\textbf{m}_{j+1} = \textbf{m}_{j} + \alpha_j \textbf{s}_j.  
\end{equation}
 The next model, $\textbf{m}_{j+1}$, is found by summing the current model, $\textbf{m}_{j}$, to some search direction, $\textbf{s}_j$, scaled by a step length, $\alpha_j$. There are many ways to compute the search direction, $\textbf{s}_j$. We use the nonlinear conjugate gradient method in which:
\begin{equation}
\textbf{s}_j=\textbf{s}_{j-1}+\beta\nabla J(\textbf{m}_j),
\end{equation}
where $\textbf{s}_{j-1}$ is the previous search direction and $\beta$ is the conjugate direction coefficient, and $\nabla J(\textbf{m}_j)$ is the gradient of the objective function at the current model. Furthermore, $B(m_j)^*$ is the adjoint of the wave equation operator linearized around the current model iteration applied to the difference between the modeled and observed data:
\begin{equation}
\nabla J(\textbf{m}_j) = - \sum_{i=1}^N B(\textbf{m}_j)^*(f_i(\textbf{m}) - \textbf{d}^{obs}_i)   
\end{equation}

To put it concisely, at each iteration of FWI we use the gradient of the objective function to to update the earth model in order to reduce the value of the objective function. We stop iterating when the objective function reaches zero or, more realistically, once it stops reducing. 

However, the nonlinearity of the FWI objective function means it is not convex with respect to the earth model. Gradient descent methods, like the one described above, will fall into a local minimum, that is find an earth model at which the objective function stops reducing but does not represent the global minimum of the objective function. In order to avoid local minima, the initial model used in the inversion scheme, $\textbf{m}_0$ must be fairly close to the true model. Herein lies one of the largest restrictions of FWI, that being we must start from an earth model that is fairly close to the true model in order for the gradient based optimization algorithm  to converge to the true solution.

As is apparent by the non-linear relationship between $d_m$ and $m$ this inversion is
nonlinear. Additionally, since reflection seismic surveys $d_{obs}$ contains
surface seismic data, it does not contain all of the necessary information to
define a earth model that varies arbitrarily with depth and along the
horizontal directions (\cite{Biondi2001}). This means that, in general, minimizing
Equation~\ref{eq:tomo} is an ill-posed problem. While in using a deep learning
approach to tomography we do not rely on numerical solutions of the Eikonal or
wave-equations. 


